MinIndy: Uma Ferramenta de In\'icio R\'apido do Hyperledger Indy

The Hyperledger Indy blockchain platform, aimed at identity management networks, has gained importance, but instantiating a complete network is complex and requires experience. Therefore, the present work describes MinIndy, a tool designed to simplify the installation and configuration of Hyperledger Indy networks. This simplification will allow people with a lower level of expertise to create their Indy networks. Which makes it a viable alternative for organizations looking to adopt Hyperledger Indy Blockchain networks with less effort.

==> i18n/brazil/appx/tutorial.tex <==
Cada um dos Trustees gera suas informações (Trustee DID and Verkey (Verification key)) usando o indy-cli.

Cada um dos Stewards (extamente 4) gera suas suas informações (Trustee DID and Verkey (Verification key)) usando o indy-cli. Os Stewards podem ter um Validator (nó pertecente a rede).

São geradas informações do Validator (Verkey, BLS )

As informações do Steards e do Trustees vão estar na tabela  os arquivos gêneses (genesis files)
Gerar as chaves do nó Validator;
Preencher a tabela para gerar os arquivos gêneses (genesis files)


% Node-stack name is Steward1
% Client-stack name is Steward1C
% Generating keys for random seed b'88c26d3C92bc33Be077Bf22FCBa60E2A'

% Init local keys for client-stack
% Public key is DGM7x7SQvjKjfUa7VLo5gGCZ6WfKASo6Cp5uP3aBRf7j
% Verification key is DJrzRm3ahRkz2pesFVtmH8wA3S3z63XayZgDvV21b4BF

% Init local keys for node-stack
% Public key is DGM7x7SQvjKjfUa7VLo5gGCZ6WfKASo6Cp5uP3aBRf7j
% Verification key is DJrzRm3ahRkz2pesFVtmH8wA3S3z63XayZgDvV21b4BF
% BLS Public key is 3k9aPxmqMYY4QQ3MK88Pot5QmqxfaaxuzMeGnKYT8j1Ds1Rcmq2zmjQmLMtKvBzC89E7yCQyiQ9HEDcGAZi6zmarMCQNkY9oYCAUVJGrZgxBE4a1oj7VYKw7zuGpMwsKLPGLcTGwpmX9LS6f5ykbazEwEgQRTiWj2epRKxZC87DLwbH
% Proof of possession for BLS key is RT5vLkN7639sXwYMBWkuFnzSM7ezEb49ZZExf6htH1WBWyuYgJsRTqT71HWaizfFLi1zp63eNGKKVzzyMaETYoj8QoV3GejHeZzP7LydJQpHQ5VPuLW3NUy5BGH4Xt7RkCT5pUbwhjz6mwxXfGAtQot7kiMH18QrpcazAmHrFPXKe7

==> i18n/brazil/sec/exp-results.tex <==
%------------------------------------------------------------
\section{Resultados Esperados} 
\label{sec:exp-results}
%------------------------------------------------------------

% * Apresentação dos resultados esperados após a realização dos experimentos
% * Discussão sobre a possível eficácia da solução proposta

% Exemplo
% O objetivo da presente pesquisa em computação é desenvolver e avaliar um novo algoritmo de compressão de imagem baseado em deep learning. Espera-se que o novo algoritmo proposto apresente um desempenho superior em relação aos métodos de compressão de imagem existentes, tanto em termos de qualidade da imagem comprimida quanto em eficiência computacional.

% Em particular, espera-se que o novo algoritmo de compressão de imagem proposto possa reduzir a taxa de bits necessária para representar uma imagem digital sem comprometer significativamente a qualidade visual da imagem. Além disso, espera-se que o algoritmo proposto seja capaz de lidar eficientemente com diferentes tipos de imagens, incluindo imagens naturais, médicas e de satélite, e seja escalável para grandes conjuntos de dados.

% Espera-se que os resultados desta pesquisa tenham um impacto significativo na área de processamento de imagens, possibilitando a criação de novas aplicações e tecnologias que dependem da compressão de imagens. Por exemplo, espera-se que o novo algoritmo possa ser usado para melhorar a eficiência de transmissão de imagens em redes de comunicação com largura de banda limitada, permitindo a transmissão de imagens de alta qualidade em tempo real.

% Por fim, espera-se que esta pesquisa possa fornecer uma base sólida para futuras investigações na área de deep learning aplicado à compressão de imagens e inspire novas abordagens para o desenvolvimento de algoritmos de compressão de imagens mais avançados e eficientes.

O objetivo da avaliação é mostrar que, apesar da redução do tempo para instanciar uma rede Indy, não há, sob as mesmas condições de ambiente, diferenças de desempenho entre uma rede Indy instanciada pelo método tradicional e uma em que se utiliza o MinIndy,  seja em termos de latência, de transações por segundo, de uso de recursos do sistema, de taxa de falhas e de taxa de transferência. Isso ocorre porque a automatização não impõe restrições sobre a rede, tão somente automatiza o processo de instanciação e configuração.  

Espera-se também que o MinIndy na prática reduza o tempo necessário para instanciar um nó da rede Indy, de modo a facilitar a conexão de novos nós a uma rede existente.

Por fim, espera-se que a ferramenta aqui apresentada possa ser usada por indivíduos e organizações interessados em instanciar uma rede Indy num primeiro momento para teste e homologação e posteriormente para produção. Além disso, espera-se que a ferramenta possa ser aprimorada ou sirva como base para desenvolver novas ferramentas de automatização de instanciação de redes Indy, ou mesmo de outros modelos de rede blockchain, como Hyperledger Besu.



==> i18n/brazil/sec/theor_bkgd.tex <==
%------------------------------------------------------------
\section{Fundamentação Teórica} 
\label{sec:theor_bkgd}
%------------------------------------------------------------

\subsection{Hyperledger Indy}

\subsubsection{Atores}

Os integrantes das redes Indy possuem dois papeis: \textit{Trustee}, que são as pessoas responsáveis por gerenciar a rede e proteger a integridade da Governança da Rede. Para uma rede de produção, são necessários no mínimo três \textit{Trustees}, ou seja, três pessoas diferentes são necessárias, e mais são preferíveis; um \textit{Steward} é uma organização responsável por executar um nó na rede. Exatamente 4 \textit{Stewards} ``Genesis'' são necessários para estabelecer um nova rede, ou seja 4 organizações diferentes, mais \textit{Stewards} podem ser adicionados posteriormente. Os \textit{Stewards} operam os nós \textit{Validator} da rede de identidade descentralizada Sovrin.

O nó \textit{Validator} será a máquina que se tornará parte de uma rede Indy. Um nó \textit{Validador} permitirá que a organização faça parte do que é chamado de consenso. Por padrão, um \textit{Steward} só tem permissão para operar um nó \textit{Validador} por rede.


% A documentação pedi que o nó Validator tenha 2 placas de rede, entretanto, é muito difícil um pequena organização tenha duas para ter 2 endereços IPs.

\subsubsection{Criação de uma Rede}

% Create DIDs for Trustees.
Os Trustees iniciais (3 preferidos) devem criar e enviar um DID (identificador descentralizado) e Verkey (Chave de Verificação) para que o arquivo de gênese do domínio possa ser construído.

% Create DIDs for Stewards
Os Stewards também deverão criar e enviar um DID e Verkey. 


% Instalação, configuração e criação de chave para o Validator.
Deverão ser criadas as informações para cada um Validators. Os Stewards também são responsáveis pelas informações dos seus respectivos Validators, como: o endereço IP e porta para comunicações entre nós, endereço e porta para conexões de cliente, pseudônimo, semente para criação das chaves, Verkey, chave pública BLS, chave de prova de posse BLS. Para isso, as seguinte etapas são necessárias:

% https://github.com/hyperledger/indy-node/blob/ubuntu-16.04/docs/source/installation-and-configuration.md
Informações Preliminares do Nó Validador
Obter os endereços IP
Seu nó Validator será a máquina que se tornará parte de uma rede Indy. Ele deve ter dois endereços IP estáticos. Ele deve ser configurado para que as conexões TCP/IP de saída sejam desses mesmos endereços, assim como as conexões de entrada.

Obtenha endereços IP que atendam a esse requisito.

Escolha os números das portas
O nó Validador também deverá ter o seguinte:

Porta do Nó: (TCP) Os validadores usam essa combinação de endereço IP e porta para se comunicarem entre si.
Porta do cliente: (TCP) Os clientes usam essa combinação de endereço IP e porta para se comunicar com o nó Validador, para interagir com o ledger.

Por convenção, as portas 9701 e 9702 são escolhidas como portas Node e Client, respectivamente.

Escolha um pseudônimo:

Seu nó Validador precisará ter um alias. Isso será usado posteriormente quando criarmos uma chave para o nó. Pode ser qualquer nome exclusivo e conveniente que você não se importe que o mundo veja. Ele não precisa fazer referência ao nome da sua empresa; no entanto, deve ser distinguível dos outros nós do Validador na rede. Muitos Stewards escolhem um pseudônimo de Validator que identifica sua organização, por orgulho de sua contribuição para a causa da identidade auto-soberana.

Instalar o nó validador
% https://github.com/hyperledger/indy-node/blob/ubuntu-16.04/docs/source/installation-and-configuration.md#322-install-the-validator-node

Crie a chave para o nó validador

IMPORTANTE: muitos provedores, como a AWS, usam endereços IP locais não roteáveis em seus nós e, em seguida, usam NAT para convertê-los em endereços IP públicos roteáveis. Se você estiver em tal sistema, use os endereços locais para o comando init_indy_node.

Execute o seguinte no Validador antes de executar init_indy_node.

No arquivo /etc/indy/indy_config.py, altere o nome da rede de “sandbox” (Sovrin StagingNet) para “net3” (Sovrin BuilderNet) (use sudo para editar o arquivo ou use sudo sed -i -re "s/ (NETWORK_NAME = ')\w+/\1net3/" /etc/indy/indy_config.py) e execute os seguintes comandos:
Observação: é aqui que você substituiria o nome do diretório da nova rede se estivesse configurando uma nova rede.

Digite o seguinte onde <ALIAS> é o alias que você escolheu para sua máquina do nó do Validador e <node ip>, <client IP>, <node port #> e <client port #> são os valores corretos para o seu Validator.

Observação: os endereços IP do nó e do cliente devem ser os endereços LOCAL do seu nó.

% ubuntu@validator$ sudo -i -u indy init_indy_node <ALIAS> <ip do nó> <porta do nó> <ip do cliente> <porta do cliente>

Você verá algo assim:

% Node-stack name is Node19
% Client-stack name is Node19C
% Generating keys for random seed b'FA7b1cc42Da11B8F4BC83990cECF63aD'
% Init local keys for client-stack
% Public key is a9abcd497631de182bb6f767ffb4921cdf83ffdb20e9d22e252883b4fc34bf2f
% Verification key is 3d604d22c4bbfd55508a5a7e0008847bdeccd98a41acd048b500030020629ee1
% Init local keys for node-stack
% Public key is a9abcd497631de182bb6f767ffb4921cdf83ffdb20e9d22e252883b4fc34bf2f
% Verification key is bfede8c4581f03d16eb053450d103477c6e840e5682adc67dc948a177ab8bc9b
% BLS Public key is 4kCWXzcEEzdh93rf3zhhDEeybLij7AwcE4NDewTf3LRdn8eoKBwufFcUyyvSJ4GfPpTQLuX6iHjQwnCCQx4sSpfnptCWzvFEdJnhNSt4tJMQ2EzjcL9ewRWi24QxAaCnwbm2BBGJXF7JjqFgMzGfuFXXHhGPX3UtdfAphrojk3A1sgq
% Proof of possession for BLS key is QqPuAnjnkYcE51H11Tub12i7Yri3ZLHmEYtJuaH1NFYKZBLi87SXgC3tMHxw3LMxErnbFwJCSdJKbTb2aCVmGzqXQtVWSpTVEQCsaSm4SUZLbzWVoHNQqDJASRYNbHH2CqpR2MtntA4YNb2WixNSZNXFSdHMbB1yMQ7XUcZqtGHhcb

Armazene o comando original, a semente aleatória, a chave de verificação, a chave pública BLS e a prova de posse (POP) da chave BLS. Estas são as chaves para o seu nó Validator (não confundir com as chaves para você em sua função de Steward). A chave de verificação do Validator e a chave BLS (com seu POP) são públicas e serão publicadas no ledger.

A semente aleatória deve ser protegida contra divulgação.

As informações dos Trustees, Stewards e Validator são utilizadas para gerar os arquivos de gênese da rede. As informações dos Trustees são utilizadas para gerar o arquivo Domain e as dos Stewards e Validator para o Pool.

% Create and Distribute genesis transaction files
Salve as planilhas preenchidas pelos curadores e administradores como arquivos separados no formato csv e use o script genesis_from_files.py para gerar os arquivos pool_transactions_genesis e domain_transactions_genesis para a rede.

Publique os arquivos genesis em um local público, como um repositório GitHub associado à sua rede. Os Administradores e usuários finais precisarão dessas informações.

Informe aos Stewards e Trustees onde eles podem baixar os arquivos do genesis.

Os curadores e administradores precisarão registrar o pool_transactions_genesis com seu indy-cli para concluir a configuração e poder se conectar à rede quando estiver em execução. Como e onde eles precisam registrar o pool_transactions_genesis depende de como eles configuram seu ambiente indy-cli; Instalando o indy-cli

Os Stewards também precisarão baixar os arquivos genesis em seus nós enquanto completam a configuração. Todas as etapas a seguir devem ser concluídas no nó.

Defina o nome da rede em /etc/indy/indy_config.py, substituindo <the_network_name> no comando a seguir pelo nome da rede real;

sudo sed -i -re "s/(NETWORK_NAME = ')\w+/\1<the_network_name>/" /etc/indy/indy_config.py

Crie um diretório de rede e baixe os arquivos do genesis nele. O nome do diretório deve ser o mesmo em todos os nós e deve corresponder ao nome da rede.

sudo -i -u indy mkdir /var/lib/indy/<the_network_name>
cd /var/lib/indy/<the_network_name>
sudo curl -o domain_transactions_genesis <url_to_the_raw_domain_transactions_genesis_file>
sudo curl -o pool_transactions_genesis <url_to_the_raw_pool_transactions_genesis_file>
sudo chown indy:indy *
É importante que os arquivos sejam de propriedade de indy:indy.

\subsubsection{Adição de um Novo Nó}


==> i18n/english/english.tex <==
\title{i18n model to \LaTeX}

\maketitle

\begin{abstract}

\end{abstract}

\input{i18n/brazil/sec/intro}

==> i18n/english/sec/abs.tex <==
This paper describes MinIndy, a a tool under development designed to facilitate the installation and configuration of Hyperledger Indy networks. To evaluate its effectiveness, a comparative performance study will be performed between MinIndy and the traditional installation method recommended by the Hyperledger Foundation. The goal of the analysis is to show that MinIndy presents equivalent performance to the conventional method, which makes it a viable alternative for organizations looking to adopt Hyperledger Indy Blockchain networks using less man-hour.

==> i18n/english/sec/intro.tex <==


%------------------------------------------------------
\section{Introduction}\label{sec:intro}
%------------------------------------------------------
